On the Statistical Evolution of the Large-scale Structure and the Effective Dynamics

In this paper, we study the statistical evolution of the large-scale structure (LSS), focusing on the joint probability distribution function (PDF) of the coarse-grained cosmic field and its role in constructing effective dynamics. As the most comprehensive statistics, this PDF encodes all cosmological information of large-scale modes, therefore, could serve as the basis in the LSS modelling. Following the so-called PDF-based method from turbulence, we write down this PDF's evolution equation, which describes the probability conservation. We show that this conservation equation's characteristic curves follow the same PDF history and could be considered as an effective dynamics of the coarse-grained field. Unlike the EFT of LSS, which conceptually would work at both realization and statistics level, this effective dynamics is valid only statistically. However, this `statistical equivalence' also provides valuable insight into scale interactions at the statistical level. It also enables predicting a wide variety of statistics beyond the typical N-point polyspectra, including, e.g. topologies, density PDF and non-linear covariance matrices etc. Our formula expresses the small-scale effect as the ensemble average of their interactions conditional on the large-scale modes. This suggests an interesting way to measure effective terms directly from simulation. By applying the Gram-Charlier expansion, we demonstrate a different structure of these effective terms. This formalism is a natural framework for discussing the evolution of statistical properties of large-scale modes, and provides an alternative view for understanding the relationship between general effective dynamics and standard perturbation theory.

==> bib.tex <==

\bibitem[]{FinCom}
The finiteness is only a convenience choice to avoid path-integral like formalism. 


\bibitem[Bardeen et al. (1986)]{BBKS86}
Bardeen, J. M., Bond, J. R., Kaiser, N., Szalay, A. S., 1986, ApJ, 304, 15


\bibitem[Baumann et al.(2012)]{BEFT12}
%Cosmological non-linearities as an effective fluid
Baumann, D., Nicolis, A., Senatore, L., \& Zaldarriaga, M.\ 2012, JCAP, 7, 051


\bibitem[Bernardeau et al.(2002)]{BCGS02}
Bernardeau, F., Colombi, S., Gazta\~{n}aga, E., Scoccimarro, R., 
2002, Physical Report, 367, 1

\bibitem[Bernardeau et al.(2008)]{BCS08}
  %``Multi-Point Propagators in Cosmological Gravitational Instability,''
Bernardeau, F., Crocce, M., Scoccimarro, R.,, 2008, Phys.\ Rev.\ D, 78, 103521




\bibitem[Carrasco et al.(2012)]{CHS12}
Carrasco, J.~J.~M., Hertzberg, M.~P.,\& Senatore, L.\ 2012, Journal of High Energy Physics, 9, 82
%The effective field theory of cosmological large scale structures


\bibitem[Crocce \& Scoccimarro(2006a)]{CS06a}
  %``Renormalized cosmological perturbation theory,''
Crocce, M.,  Scoccimarro, R., 2006,  Phys.\ Rev.\ D,  73, 063519


\bibitem[Crocce \& Scoccimarro(2006b)]{CS06b}
%``Memory of initial conditions in gravitational clustering,''
Crocce, M.,  Scoccimarro, R., 2006,  Phys.\ Rev.\ D,  73, 063520



\bibitem[Kendall(1958)]{Ken1958}
Kendall M. G., Stuart A., 1958, The Advanced Theory of Statistics. Vol. 1, Griffin, London

\bibitem[Kofman \& Pogosyan (1995)]{KP95}
Kofman, L., Pogosyan, D. Yu. 1995, ApJ, 442, 30

\bibitem[Kundt \& Tr\"{u}mper (1961)]{KT61}
Kundt, W., Tr\"{u}mper, M. 1961, Akad. Wiss. Lit. Mainz Abh. Math.-Nat.
Kl., 12

%\bibitem[Lacey \& Cole (1993)]{LC93}
%Lacey, C., Cole, S., 1993, MNRAS, 262, 627

\bibitem[Lemson \& Kauffmann (1999)]{LK99}
Lemson G., Kauffmann G., 1999, MNRAS, 302, 111

\bibitem[Lesame et al. (1995)]{LDE95}
Lesame, W. M., Dunsby, P. K. S., Ellis, G. F. R., 1995, Phys. Rev. D, 52, 3406


\bibitem[Ma (1985)]{Ma85}
Ma, S. K., 1985, Statistical Mechanics (Philadelphia: World Scientific)

%\bibitem[Ma \& Bertschinger (2004)]{MB04}
%Ma, C., Bertschinger, E., 2004, ApJ, 612, 28


\bibitem[Macci\`{o} et al. (2007)]{MD07}
Macci\`{o} A. V., Dutton A. A., van den Bosch F. C., Moore B., Potter D., Stadel
J., 2007, MNRAS, 378, 55

%\bibitem[Maggiore \& Riotto (2010a)]{MR10a}
%Maggiore, M., Riotto, A., 2010, ApJ, 711, 907

\bibitem[Maggiore \& Riotto (2010b)]{MR10b}
Maggiore, M., Riotto, A., 2010, ApJ, 717, 515


\bibitem[Matarrese et al. (1993)]{MPS93}
Matarrese, S., Pantano, O., Saez, D., 1993, Phys. Rev. D., 47, 1311

\bibitem[Matarrese (1994)]{MPS94}
Matarrese, S., Pantano, O., Saez, D., 1994, Phys. Rev. Lett., 72, 320


\bibitem[Matsubara(1994)]{Mat1994}
Matsubara, T.\ 1994, ApJL, 434, L43
%Analytic expression of the genus in a weakly non-Gaussian field induced by gravity

\bibitem[Matsubara (2003)]{Mat03}
Matsubara, T., 2003, ApJ, 584, 1

\bibitem[Matsubara(2008a)]{M08a}
  %``Resumming Cosmological Perturbations via the Lagrangian Picture: One-loop Results in Real Space and in Redshift Space,''
Matsubara, T., 2008, Phys.\ Rev.\ D,  77, 063530

%\bibitem[Mo \& White (1996)]{MW96}
%Mo, H., J., White, S., D., M., 1996, MNRAS, 282, 347


\bibitem[Mercolli \& Pajer(2014)]{MP14}
%On the Velocity in the Effective Field Theory of Large Scale Structures
Mercolli, L., \& Pajer, E.\ 2014, JCAP, 3, 006


\bibitem[Neyman \& Scott (1952)]{NS52}
Neyman J., Scott E. L., 1952, Astrophys. J. 116, 144

\bibitem[Neyrinck et al. (2009)]{NSS09}
Neyrinck, M. C., Szapudi, I., Szalay, A. S., 2009, ApJ, 698L, 90

\bibitem[Neyrinck et al. (2011)]{NSS11}
Neyrinck, M. C., Szapudi, I., Szalay, A. S., 2011, ApJ, 731, 116


\bibitem[Ohkitani \& Kishiba (1995)]{OK95}
Ohkitani, K., Kishiba, S., 1995, Phys. Fluids, 7, 411


\bibitem[Pajer \& Zaldarriaga(2013)]{PZ13}
Pajer, E., \& Zaldarriaga, M.\ 2013, JCAP, 8, 037
%On the renormalization of the effective field theory of large scale structures

\bibitem[Peebles (1980)]{P80}
Peebles P. J. E., 1980, The large-scale structure of the universe, Peebles, P. J. E., ed.

\bibitem[Pietroni(2008)]{P08}
  %``Flowing with Time: a New Approach to Nonlinear Cosmological Perturbations,''
Pietroni, M., 2008, JCAP, 0810, 036

\bibitem[Pogosyan et al.(2009)]{PGP09}
Pogosyan, D., Gay, C., \& Pichon, C.\ 2009, PRD, 80, 081301
%Invariant joint distribution of a stationary random field and its derivatives: Euler characteristic and critical point counts in 2 and 3D

\bibitem[Pope (1985)]{Pop85}
%PDF methods for turbulent reactive flows
Pope, S. B., Progress in Energy and Combustion Science, 1985, 11, 119

\bibitem[Press \& Schechter (1974)]{PS74}
Press, W., Schechter, P., 1974, ApJ, 187, 425

\bibitem[Pueblas \& Scoccimarro (2009)]{PS09}
Pueblas, S., Scoccimarro, R., 2009, Phys. Rev. D, 80, 043504


\bibitem[Sheth (1998)]{Sh98}
Sheth, R., K., 1998, MNRAS, 300, 1057

\bibitem[Sheth \& Tormen (2002)]{ST02}
Sheth R. K., Tormen G., 2002, MNRAS, 329, 61

\bibitem[Sheth \& Tormen (2004)]{ST04}
Sheth R. K., Tormen G., 2004, MNRAS, 350, 1385


\bibitem[Taruya \& Hiramatsu(2008)]{TH08}
  %``A Closure Theory for Non-linear Evolution of Cosmological Power Spectra,''
Taruya, A., Hiramatsu, T., 2008,  ApJ, 674, 617 


\bibitem[Wang et al. (2014)]{WS14}
Wang, X., Szalay, A., Aragón-Calvo, M. A., Neyrinck, M. C., Eyink, G. L., 
2014, ApJ, 793, 58


\bibitem[Wechsler et al. (2005)]{WZ05}
Wechsler R. H., Zentner A. R., Bullock J. S., Kravtsov A. V., Allgood B.,
2005, ApJ, 652, 71


\bibitem[Wetzel et al. (2007)]{WCW07}
Wetzel A. R., Cohn J. D., White M., Holz D. E., Warren M. S., 2007, ApJ,
656, 139
%

\bibitem[Zel'dovich (1970)]{ZA70}
Zel'dovich, Ya. B., 1970, Astronomy and Astrophysics, 5, 84

